FairRelay: Fair and Cost-Efficient Peer-to-Peer Content Delivery through Payment Channel Networks

Peer-to-Peer (P2P) content delivery, known for scalability and resilience, offers a decentralized alternative to traditional centralized Content Delivery Networks (CDNs). A significant challenge in P2P content delivery remains: the fair compensation of relayers for their bandwidth contributions. Existing solutions employ blockchains for payment settlements, however, they are not practical due to high on-chain costs and over-simplified network assumptions. In this paper, we introduce FairRelay, a fair and cost-efficient protocol that ensures all participants get fair payoff in complex content delivery network settings. We introduce a novel primitive, Enforceable Accumulative Hashed TimeLock Contract (Enforceable A-HTLC), designed to guarantee payment atomicity - ensuring all participants receive their payments upon successful content delivery. The fairness of FairRelay is proved using the Universal Composability (UC) framework. Our evaluation demonstrates that, in optimistic scenarios, FairRelay employs zero on-chain costs. In pessimistic scenarios, the on-chain dispute costs for relayers and customers are constant, irrespective of the network complexity. Specifically, empirical results indicate that the on-chain dispute costs for relayers and customers are 24,902 gas (equivalent to 0.01 USD on Optimism L2) and 290,797 gas (0.07 USD), respectively. In a 10-hop relay path, FairRelay introduces less than 1.5% additional overhead compared to pure data transmission, showcasing the efficiency of FairRelay.

==> img_texs/intro_model.tex <==
\begin{figure}[htp]
    \centering
    \includegraphics[width=0.4\textwidth]{draft_v1/imgs/intro_model.pdf}
    \caption{A digital content delivery process with multiple relay pathways succeeds only if all relay are paid fees.}
    \label{fig:intro_model}
\end{figure}

==> img_texs/lock_path.tex <==
\begin{figure}[htbp]
    \centering
    \includegraphics[width=0.47\textwidth]{imgs/lock_path.pdf}
    \caption{Enforceable A-HTLC Workflow}
    \label{fig:lock_path}
\end{figure}

==> tabs/simp_related_tab.tex <==
\begin{table*}[htbp]
    \resizebox{\textwidth}{!}{%
    \begin{tabular}{c|ccccc|c}
        \hline
        \textbf{Features} & FairSwap & CacheCash & Gringotts & FairDownload & Bitstream & Our protocol \\
        Multi-relay &\color[HTML]{9B9B9B}\xmark &\color[HTML]{009901}\checkmark&\color[HTML]{009901}\checkmark&\color[HTML]{009901}\checkmark&\color[HTML]{9B9B9B}\xmark & \color[HTML]{009901}\cmark \\
        Multi-hop & \color[HTML]{9B9B9B}\xmark & \color[HTML]{9B9B9B}\xmark & \color[HTML]{9B9B9B}\xmark & \color[HTML]{9B9B9B}\xmark & \color[HTML]{9B9B9B}\xmark & \color[HTML]{009901}\cmark \\
        Customer Fairness & \color[HTML]{009901}\checkmark & - & \color[HTML]{009901}\checkmark & \color[HTML]{009901}\checkmark & \color[HTML]{009901}\checkmark & \color[HTML]{009901}\cmark \\
        Relay Fairness & - & \color[HTML]{009901}\checkmark & \color[HTML]{009901}\checkmark & \color[HTML]{009901}\checkmark & - & \color[HTML]{009901}\cmark \\
        Provider Fairness & \color[HTML]{009901}\checkmark & \color[HTML]{9B9B9B}\xmark & \color[HTML]{9B9B9B}\xmark & \color[HTML]{009901}\checkmark & \color[HTML]{009901}\checkmark & \color[HTML]{009901}\cmark \\
        Confidentiality & \color[HTML]{009901}\checkmark & \color[HTML]{9B9B9B}\xmark & \color[HTML]{9B9B9B}\xmark & \color[HTML]{009901}\checkmark & \color[HTML]{009901}\checkmark & \color[HTML]{009901}\cmark \\
        \hline
        Bandwidth Free-riding & all chunks' & all chunks' & multiple chunks' & One chunk's & all chunks' & \textbf{one packet's} \\
        Optimistic Cost & $O(1)$ & $O(n)$ & $O(n)$ & O(x) & 0 & \textbf{0} \\
        Pessimistic Cost & $O(1)$ & $O(n)$ & $O(n)$ & O(x) & $O(1)$ & $\textbf{O(x)}$ \\
        \hline
    \end{tabular}%
    }
    \caption{\textbf{Comparing different decentralized content delivery protocols.} "x" denotes the number of relays.}
    \label{tab:simp_related}
\end{table*}
